Consistent Causal Inference of Group Effects in Non-Targeted Trials with Finitely Many Effect Levels

A treatment may be appropriate for some group (the ``sick" group) on whom it has a positive effect, but it can also have a detrimental effect on subjects from another group (the ``healthy" group). In a non-targeted trial both sick and healthy subjects may be treated, producing heterogeneous effects within the treated group. Inferring the correct treatment effect on the sick population is then difficult, because the effects on the different groups get tangled. We propose an efficient nonparametric approach to estimating the group effects, called {\bf PCM} (pre-cluster and merge). We prove its asymptotic consistency in a general setting and show, on synthetic data, more than a 10x improvement in accuracy over existing state-of-the-art. Our approach applies more generally to consistent estimation of functions with a finite range.

==> NotationMacros.tex <==
%%%
%%% superscript: with () unless denoting power
%%% vector: bold small face
%%% matrix: ROMAN capital face
%%% summation: iterator same small face (e.g., n), range capital face (e.g., N)
%%%            use i, j only in double-summation
%%% log: use ln for natural log

\newcommand{\supstar}{^{\raisebox{-2pt}{\hspace*{-0.8pt}{\tiny \textsc{*}}}}}

%we introduce some macro commands for this notation.
\newcommand{\mat}[1]{{\ensuremath{\mathrm{#1}}}}
\newcommand{\vect}[1]{{\ensuremath{\mathbf{#1}}}}
\newcommand{\ket}[1]{{\ensuremath{|#1\rangle}}}
\newcommand{\bra}[1]{{\ensuremath{\langle#1|}}}
\newcommand{\braket}[2]{{\ensuremath{\langle#1|#2\rangle}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Set notation
%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\set}[1]{\cl{#1}}
\def\power{\cl{P}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Letters, upper and lower
%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\w}{\ensuremath{w}}
\newcommand{\x}{\ensuremath{x}}
\def\aa{\vect{a}}
\newcommand{\bb}{\vect{b}}
\newcommand{\cc}{\vect{c}}
\newcommand{\ee}{\vect{e}}
\newcommand{\pp}{\vect{p}}
\newcommand{\qq}{\vect{q}}
\newcommand{\rr}{\vect{r}}
\newcommand{\xx}{\vect{x}}
\newcommand{\xofnofi}[2]{\x_{#1#2}}
\newcommand{\zofnofi}[2]{\z_{#1#2}}
\newcommand{\xni}{\xofnofi{n}{i}}
\newcommand{\xnj}{\xofnofi{n}{j}}
\newcommand{\zni}{\zofnofi{n}{i}}
\newcommand{\znj}{\zofnofi{n}{j}}
\newcommand{\uu}{\vect{u}}
\newcommand{\y}{\ensuremath{y}}
\newcommand{\yy}{\vect{y}}
\newcommand{\z}{\ensuremath{z}}
\newcommand{\zz}{\vect{z}}
\newcommand{\eepsilon}{\ensuremath{\boldsymbol\epsilon}}
\newcommand{\bfepsilon}{\eepsilon}

\newcommand{\vv}{\ensuremath{\mathbf{v}}}
\newcommand{\hatvv}{\ensuremath{\hat{\vv}}}

\def\D{{\cl D}}
\def\K{{\cl K}}
\def\L{{\cl L}}
\def\S{{\cl S}}
\def\X{{\cl X}}
\def\Y{{\cl Y}}

\DeclareMathSymbol{\N}{\mathbin}{AMSb}{"4E}
\DeclareMathSymbol{\Z}{\mathbin}{AMSb}{"5A}
\DeclareMathSymbol{\R}{\mathbin}{AMSb}{"52}
\DeclareMathSymbol{\Q}{\mathbin}{AMSb}{"51}
\DeclareMathSymbol{\I}{\mathbin}{AMSb}{"49}
\DeclareMathSymbol{\C}{\mathbin}{AMSb}{"43}

\newcommand{\sN}{\ensuremath{\textsc{n}}}
\newcommand{\sQ}{\ensuremath{\textsc{q}}}

%%%%%%%%%%%%%%%%%%%%%%
% Useful Quantities
%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dvc}{\ensuremath{d_{\textsc{vc}}}}
\newcommand{\vcd}{\ensuremath{{d_{\textsc{vc}}}}}
%two versions of the VC dimension

%\newcommand{\dotprod}[2]{\ensuremath{#1 \;{\scriptscriptstyle \stackrel{\bullet}{{}}}\; #2}}
\newcommand{\dotprod}{\ensuremath{\;{\scriptscriptstyle \stackrel{\bullet}{{}}}\;}}
%dot product

\newcommand{\bool}[1]{\ensuremath{\left\llbracket#1\right\rrbracket}}
%boolean evaluation

\newcommand{\sign}{\ensuremath{\textrm{sign}}}
\newcommand{\poly}{\ensuremath{\textrm{poly}}}
\newcommand{\rank}{\ensuremath{\textrm{rank}}}
%sign function

\newcommand{\transp}{\ensuremath{^{\text{\textsc{t}}}}}
\newcommand{\trace}{{\textrm{\textup{trace}}}}
%transpose

\newcommand{\pinv}{\ensuremath{^{-1}}}
%pseudo inverse

\newcommand{\grad}{\ensuremath{\mathbf{g}}}
%gradient

\newcommand{\hess}{\ensuremath{\mathrm{H}}}
%Hessian

\newcommand{\DELTA}{\ensuremath{\mbox{\small $\Delta$}}}
%as in delta w

%%%
%%% Error Terms
%%%
%%% will use the same ``error'' for all kinds of errors 
%%% (classification, regression, etc.)

\newcommand{\E}{\ensuremath{E}} 
\newcommand{\Ein}{\ensuremath{E_{\textrm{\textup{in}}}}}
%in-sample error:                                  
%no subscripts to make \Ein_1, \Ein_2, ... possible.
%see \Eval, \Eoff below

\newcommand{\Eout}{\ensuremath{E_{\textrm{\textup{out}}}}}
%out-of-sample error

\newcommand{\Etest}{\ensuremath{E_{\textrm{\textup{test}}}}}
%test error (on a test set)

\newcommand{\Eaug}{\ensuremath{E_{\textrm{\textup{aug}}}}}
%the objective function: term to be minimized, including regularization

\newcommand{\Eval}{\ensuremath{E}_{\textrm{\textup{val}}}}
%validation error

\newcommand{\Eoff}{\ensuremath{E}_{\textrm{\textup{off}}}}
%off-training-set error

%\newcommand{\insample}{in-sample} %removed; just type
%for use in ``in-sample'' (training) error

%\newcommand{\outofsample}{out-of-sample} %removed; just type
%for use in ``out-of-sample'' (test) error

%%%
%%% Probability and Expectations
%%% ``probability distribution'' is generic for measure over probability space
%%%

\def\rand{\text{rand}}

\DeclareMathSymbol{\Prob}{\mathord}{AMSb}{"50}
\newcommand{\ProbOf}[1]{\Prob\!\left(#1 \right)}
\newcommand{\ProbGiven}[2]{\ProbOf{#1\ \vrule\ #2}}
\newcommand{\prob}{\ensuremath{P}}
%\newcommand{\Exp}{\ensuremath{\mathbb{E}}}
\DeclareMathSymbol{\Exp}{\mathord}{AMSb}{"45}
%expectated value
%generally, \expected_x, \expected_{x | y}, 
%but can be omitted if obvious from argument

\newcommand{\rv}[1]{\ensuremath{\mathbf#1}}
\def\rvI{\rv{I}}
\def\rvR{\rv{R}}
\def\rvU{\rv{U}}
\def\rvV{\rv{V}}
\def\rvW{\rv{W}}
\def\rvX{\rv{X}}
\def\rvY{\rv{Y}}
\def\rvZ{\rv{Z}}
\def\rvDelta{\ensuremath{\bm{\Delta}}}


%probability, of a point
%           , of an event
%           , of a density at a point
%generally, \prob_x, \prob_{x | y}, 
%but can be omitted if obvious from argument


%%%
%%% Data and Functions
%%%

% shorthand for script B notation
\newcommand{\B}{\ensuremath{\mathcal{B}}}

\newcommand{\dset}{\mathcal{D}}
%data set/training set
%can be \dset_{tr} \dset_{val} when describing validation

\newcommand{\inputspace}{\ensuremath{\mathcal{X}}}
%input space

\newcommand{\outputspace}{\ensuremath{\mathcal{Y}}}
%output space

\newcommand{\zspace}{\ensuremath{\mathcal{Z}}}
%Z space (nonlinear transformation)

\newcommand{\trans}{\ensuremath{\Phi}}
\newcommand{\transdim}{\ensuremath{\tilde d}}
\newcommand{\subtransdim}{\tilde{d}}
\newcommand{\transspace}{\ensuremath{\mathcal{Z}}}
%transformed space

\newcommand{\target}{\ensuremath{f}}
%target function

\newcommand{\hset}{\ensuremath{\mathcal{H}}}
\newcommand{\lmodel}{\ensuremath{\mathcal{L}}}
\newcommand{\lalg}{\ensuremath{\mathcal{A}}}
%hypothesis set, learning model, learning algorithm
%decide to use ``learning model'' in a new way: 
%hypothesis set + learning algorithm

%\newcommand{\hparam}{\ensuremath{\theta}}
%not using hypothesis parameter

\newcommand{\hypothesis}{\textbf{deprecated, please use hypo instead}}
\newcommand{\hypo}{\ensuremath{h}}
%hypothesis within \hset

\newcommand{\hypofinal}{\ensuremath{g}}
%final hypothesis produced

\newcommand{\hypobydset}{\ensuremath{g}^{(\dset)}}
%final hypothesis produced from a specific data set
%(in bias-variance decomposition)

\newcommand{\weakhset}{\ensuremath{\tilde{\hset}}}
%the chosen weak hypotheses set (in boosting)

\newcommand{\weakhypo}{\ensuremath{\tilde{\hypo}}}
%the chosen weak hypothesis

%%%
%%% some numbers
%%%
%Numbers

\def\0{{\bm{0}}}	%Zero vector

%Removed. Simply type n and N
%\newcommand{\Nex}{\ensuremath{N}}
%\newcommand{\iex}{\ensuremath{n}}
%\newcommand{\Nexample}{\Nex}
%number of examples

%Removed. Simply type t and T
%\newcommand{\Nit}{\ensuremath{T}}
%\newcommand{\iit}{\ensuremath{t}}
%\newcommand{\Niter}{\Nit}
%number of iterations: boosting

%Removed. Simply type t and T
%\newcommand{\Nep}{\Niter}
%\newcommand{\iep}{\Niter}
%\newcommand{\Nepoch}{\Nep}
%number of epochs: NNet, decide to reuse \Niter

%Removed. Simply type i and d
%\newcommand{\Ndim}{\ensuremath{d}}
%\newcommand{\idim}{\ensuremath{i}}
%number of dimensions

%Removed. Simply type i, j, k
%\newcommand{\ione}{\ensuremath{i}}
%\newcommand{\itwo}{\ensuremath{j}}
%generic running index

\newcommand{\Nhypo}{M}
%number of hypotheses: not decided yet
%can be M but M may also be taken in other parts

%%%
%%% input/output
%%% input will be simply called ``input''
%%% output will be simply called ``output''

%\newcommand{\xxof}[1]{\x_{1}}
%\newcommand{\xxsubof}[2]{\x_{#1#2}}
%\newcommand{\zzof}[1]{\z[#1]}
%\newcommand{\zzsubof}[2]{\z_{#1#2}}
%\newcommand{\xxni}{\xxsubof{n}{i}}
%\newcommand{\xxnj}{\xxsubof{n}{j}}
%\newcommand{\zzni}{\zzsubof{n}{i}}
%\newcommand{\zznj}{\zzsubof{n}{j}}

%input, the bold one for vector, the normal one for scalar, 
%use \x_n or \xx_n to mean the n-th input vector x_n
%\xxsubof{n}{d} intends to describe the d-th component of input vector x_n
%output, will use \y_n

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Notation specific to learning models.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%
%%% NNet
%%%

\newcommand{\bias}{\ensuremath{b}}
%bias (in perceptron, SVM, etc.)

% symbols for the nonlinearity (hard or soft threshold), which was originally S, and for the signal which was denoted briefly as x.
\newcommand{\thresh}{\ensuremath{\theta}}
\newcommand{\logistic}{\sig}
%\newcommand{\sig}{\ensuremath{{\sf sigmoid}}}
\newcommand{\sig}{\ensuremath{\theta}}
\newcommand{\signal}{\ensuremath{s}}
%signal (in neuron)

\newcommand{\activation}{\ensuremath{\theta}}
%activation (for neuron)

\newcommand{\weight}{\ensuremath{\mathbf{w}}}
\newcommand{\ww}{\vect{w}}
%weight (NNet: w_{ij}^{(\ell)})

\newcommand{\regu}{\ensuremath{\lambda}}
%regularization parameter

%%%
%%% boosting
%%%

\newcommand{\exampleweight}{\ensuremath{p}}
%weight on example, say, \exampleweight_n^{(t)}

\newcommand{\hypoweight}{\ensuremath{w}}
%weight on hypothesis

\newcommand{\werr}[1]{\ensuremath{E_{#1}}}
%weighted error (say, in the t-th iteration)

%%%
%%% SVM
%%% \xi, \lambda

\newcommand{\kernel}{\ensuremath{K}}
%kernel K(u, v) mostly

\newcommand{\bigC}{\ensuremath{C}}
%SVM: cost parameter

\newcommand{\margin}{\ensuremath{\Delta}}

\newcommand{\dualvar}{\ensuremath{\alpha}}

\providecommand\remove[1]{}
\def\Hoeffding{Generalization}
\def\Var{{\textrm{Var}}}
\def\Cov{{\textrm{Cov}}}
\def\var{{\text{\sf var}}}
\def\bias{{\text{\sf bias}}}
\def\Neff{{N_{\textrm{eff}}}}
\def\matA{\mat{A}}
\def\matB{\mat{B}}
\def\matC{\mat{C}}
\def\matD{\mat{D}}
\def\matE{\mat{E}}
\def\matH{\mat{H}}
\def\matI{\mat{I}}
\def\matP{\mat{P}}
\def\matQ{\mat{Q}}
\def\matR{\mat{R}}
\def\matS{\mat{S}}
\def\matT{\mat{T}}
\def\matU{\mat{U}}
\def\matV{\mat{V}}
\def\matW{\mat{W}}
\def\matX{\mat{X}}
\def\matY{\mat{Y}}
\def\matZ{\mat{Z}}
\def\wperp{\ww_{\perp}}
\def\win{\ww_{\textrm{\textup{lin}}}}
\def\wreg{\ww_{\textrm{\textup{reg}}}}
\def\wtarg{\ww_{\textrm{f}}}

\newcommand{\pla}{\textrm{\tiny PLA}}
\newcommand{\lin}{\textrm{lin}}

\providecommand{\hatEout}{\ensuremath{\hat{E}_{\textrm{out}}}}
\newcommand{\smallminus}{{\rule{3pt}{0.3pt}}}
\newcommand{\supminus}{^{\raisebox{2pt}{\hspace*{-0.3pt}\smallminus}}}
\newcommand{\capsupminus}{^{\protect\raisebox{0.8pt}{\hspace*{-0.4pt}\protect\rule{3pt}{0.3pt}}}}
\newcommand{\cvsupminus}{^{\protect\raisebox{3.8pt}{\hspace*{-0.4pt}\protect\rule{3pt}{0.3pt}}}}
\def\matH{\mat{H}}
\def\Var{{\textrm{Var}}}
\def\Cov{{\textrm{Cov}}}
\def\var{{\text{\sf var}}}
\def\bias{{\text{\sf bias}}}
\def\deff{{d_{\textrm{eff}}}}
\def\Neff{{N_{\textrm{eff}}}}
\def\leg{{L}}
\def\lagrange{{\cl L}}
\def\normal{{N}}
\def\wperp{\ww_{\perp}}
\def\wtarg{\ww_{\textrm{f}}}
\def\ff{\vect{\target}}
\def\matA{\mat{A}}
\def\matI{\mat{I}}
\def\matSig{\mat{\Sigma}}
\def\matGam{\mat{\Gamma}}
\def\ourindent{{\hspace*{0.25in}}}
\def\Egen{E_{\textrm{gen}}}
\def\Etr{E_{\textrm{tr}}}
\def\Eval{E_{\textrm{val}}}
\def\Sval{\sigma_{\textrm{val}}}
\def\Ecv{{E_{\textrm{cv}}}}
\def\Eoutcv{{\bar E_{\textrm{out}}}}
\def\Dtr{{\dset_{\textrm{train}}}}
\def\Dval{{\dset_{\textrm{val}}}}
\def\vhat{{\mathbf v}}
\def\g{{\mathbf g}}

% symbols for the nonlinearity (hard or soft threshold), which was originally S, and for the signal which was denoted briefly as x.
\def\thresh{{\theta}}
\def\signal{{s}}


%new symbol for pointwise error
\def\err{{\textsf{err}}}


%Notation for Number Theory
\def\Primes{{\textsc{P}}}
\def\order{\text{order}}


%Notation for Theory of Computation
\def\EXP{{\sf EXP}}
\def\P{{\sf P}}
\def\NP{{\sf NP}}
\def\coNP{{\sf co-NP}}
\def\NPcomplete{{\sf NP-complete}}
\def\sat{{\textsc{sat}}}
\def\checkmark{\text{\ding{51}}}
\def\xmark{\text{\ding{56}}}
\def\ev{\textsc{e}}

%Propositional Logic
\def\every{\textsc{every}}
\def\lfdif{\textsc{if}}
\def\lfdthen{\textsc{then}}
\def\OR{\ensuremath{\vee}}
\def\AND{\ensuremath{\wedge}}
\def\NOT{\textsc{not}}
\def\imp{\rightarrow}
\def\iff{\leftrightarrow}
\def\T{\textsc{t}}
\def\F{\textsc{f}}
\def\lequiv{\mathop{\buildrel\text{eqv}\over \equiv}}

%Strings
%\def\concat{{\raisebox{1.25pt}{\scalebox{0.75}{\math{\,\circ\,}}}}}
\def\concat{{\raisebox{1.25pt}{\scalebox{0.75}{\math{\,\bullet\,}}}}}
%\newcommand{\concatp}[1]{^{\raisebox{0.6pt}{$\scriptstyle #1$}}\raisebox{0.65pt}{\makebox[0pt][l]{\hspace*{-4pt}\scalebox{0.65}{\math{\circ}}}}\,}
\newcommand{\concatp}[1]{^{\bullet #1}}
\newcommand{\otimesp}[1]{^{\otimes #1}}
%\newcommand{\concatp}[1]{^{\scriptstyle\begin{array}{l}#1\\\circ\end{array}}}

%Number Theory
\def\lcm{\text{lcm}}

%Complexity
\def\hard{{\sc [hard]}}
\def\easy{{\sc [easy]}}

%From ch01:
\def\ebola{\textsc{ebola}}
\def\male{\textsc{male}}
\def\female{\textsc{female}}
\def\true{\textsc{true}}
\let\emptyset\varnothing

%Theory of Computing
\def\Lroot{\L_{\text{root}}}
\def\Lprime{\L_{\text{prime}}}
\def\Lpush{\L_{\text{push}}}
\def\Ldoor{\L_{\text{door}}}
\def\Lpal{\L_{\text{pal}}}
\def\Lpuncpal{\L_{\text{punc-pal}}}
\def\Lpath{\L_{\text{path}}}
\def\Lequal{\L_{\text{equal}}}
\def\Lbal{\L_{\text{bal}}}
\def\Lempty{\L_{\text{empty}}}
\def\LTM{\L_{\textsc{tm}}}
\def\Ldiag{\L_{\textsc{diag}}}
\def\LTMLB{\L_{\textsc{tm-lb}}}
\def\LDFA{\L_{\textsc{dfa}}}
\def\LCFG{\L_{\textsc{cfg}}}
\def\LZTM{\L_{\textsc{tm-00}}}
\def\LZDFA{\L_{\textsc{dfa-00}}}
\def\LZCFG{\L_{\textsc{cfg-00}}}
\def\LEMTM{\L_{\textsc{empty-tm}}}
\def\LEMDFA{\L_{\textsc{empty-dfa}}}
\def\LEMCFG{\L_{\textsc{empty-cfg}}}
\def\LEQTM{\L_{\textsc{eq-tm}}}
\def\LEQDFA{\L_{\textsc{eq-dfa}}}
\def\LEQCFG{\L_{\textsc{eq-cfg}}}
\def\LATM{\L_{\textsc{all-tm}}}
\def\LADFA{\L_{\textsc{all-dfa}}}
\def\LACFG{\L_{\textsc{all-cfg}}}
\def\LFTM{\L_{\textsc{finite-tm}}}
\def\LFDFA{\L_{\textsc{finite-dfa}}}
\def\LFCFG{\L_{\textsc{finite-cfg}}}
\def\LDTM{\L_{\textsc{tm-decider}}}
\def\LREGTM{\L_{\textsc{reg-tm}}}
\def\LCFGTM{\L_{\textsc{cfg-tm}}}
\def\LPTM{\L_{\textsc{P-tm}}}

\def\EQTM{EQ_{\textsc{tm}}}
\def\LTMEXP{\L_{\textsc{exp}}}
\def\LPCP{\L_{\textsc{pcp}}}
\def\LHW{\L_{\textsc{hw}}}
\def\Lhalt{\L_{\textsc{halt}}}
\def\LEQ{\L_{\textsc{eq}}}
\def\UTM{U_{\textsc{tm}}}
\def\HTM{H_{\textsc{tm}}}
\def\HLB{H_{\textsc{lb}}}
\def\ETM{E_{\textsc{tm}}}
\def\ATM{A_{\textsc{tm}}}
\def\ALB{A_{\textsc{lb}}}
\def\AZTM{A_{\textsc{tm-00}}}
\def\ADTM{A_{\textsc{tm-decider}}}
\def\APTM{A_{\textsc{P-tm}}}
\def\DTM{D}
\def\HWTM{HW_{\textsc{tm}}}
\newcommand{\yesbox}{\begin{tikzpicture}[font=\small,baseline=-2.5pt]
\node[draw,inner sep=2pt,rounded corners=3pt] at (-1,0){\textsc{yes}};\end{tikzpicture}}
\def\nobox{\tikz[font=\small,baseline=-2.5pt]{
\node[draw,inner sep=2pt,rounded corners=3pt] at (-1,0){\textsc{no}};}}
\def\yesboxshade{\tikz[font=\small,baseline=-2.5pt]{
\node[draw,inner sep=2pt,rounded corners=3pt,fill=fillLightgray] at (-1,0){\textsc{yes}};}}
\def\noboxshade{\tikz[font=\small,baseline=-2.5pt]{
\node[draw,inner sep=2pt,rounded corners=3pt,fill=fillLightgray] at (-1,0){\textsc{no}};}}
\newsavebox\YN
\begin{lrbox}{\YN}
\yesbox{} or \nobox{}
\end{lrbox}
\newsavebox\YBOX
\begin{lrbox}{\YBOX}
\yesbox{}
\end{lrbox}
\newsavebox\NBOX
\begin{lrbox}{\NBOX}
\nobox{}
\end{lrbox}
\def\grammar{\textsc{cfg}}
\def\produces{\mathop{
    \tikz[baseline=-6pt]{
      \node[scale=1,inner sep=-1pt](s)at(0,0){\math{*}};
      \node[scale=1,inner sep=0pt](a)at($(s)+(0.065,-0.15)$){\math{\Rightarrow}};
    }}}
%\def\produces{\mathop{\Rightarrow^{\hspace*{-9pt}\textstyle*\hspace*{4pt}}}}
\def\eof{\textsc{eof}}
\def\markone{\raisebox{1pt}{\scriptsize\math{\begin{array}{c}\green{\checkmark}\\[-4pt]\hspace*{2pt}1\hspace*{-2pt}\end{array}}}}
\def\markzero{\raisebox{1pt}{\scriptsize\math{\begin{array}{c}\green{\checkmark}\\[-4pt]\hspace*{2pt}0\hspace*{-2pt}\end{array}}}}
\def\markredone{\raisebox{1pt}{\scriptsize\math{\begin{array}{c}\red{\xmark}\\[-4pt]\hspace*{2pt}1\hspace*{-2pt}\end{array}}}}
\def\markredzero{\raisebox{1pt}{\scriptsize\math{\begin{array}{c}\red{\xmark}\\[-4pt]\hspace*{2pt}0\hspace*{-2pt}\end{array}}}}
\def\markzeroone{\raisebox{1pt}{\scriptsize\math{\begin{array}{c}\green{\hspace*{3pt}\checkmark}\\[-3pt]\hspace*{0pt}0,\!\!1\hspace*{-2pt}\end{array}}}}
\newcommand{\encode}[1]{\langle #1 \rangle}
\def\leR{\le_{\hspace*{0pt}\textsc{r}}}
\def\leP{\le_{\hspace*{0pt}\textsc{p}}}

\def\punct{\texttt{\#}}
\def\sp{\text{\tt\textvisiblespace}}


%Proofs and Proof Templates
\newcounter{prooftemplatenum}
\setcounter{prooftemplatenum}{1}
\def\prooftempnum{{\RN{\theprooftemplatenum}}\addtocounter{prooftemplatenum}{1}}

%Directed Graphs
\def\outdeg{\text{out-deg}}
\def\indeg{\text{in-deg}}
\def\de{\hspace*{-2.75pt}\rightarrow\hspace*{-2.75pt}}

%Gates
\def\cnot{\ensuremath{^C\textsc{not}}}
\def\measure{\ensuremath{\bm{?}}}

